On the Accessibility and Controllability of Statistical Linearization for Stochastic Control: Algebraic Rank Conditions and their Genericity

Statistical linearization has recently seen a particular surge of interest as a numerically cheap method for robust control of stochastic differential equations. Although it has already been successfully applied to control complex stochastic systems, accessibility and controllability properties of statistical linearization, which are key to make the robust control problem well-posed, have not been investigated yet. In this paper, we bridge this gap by providing sufficient conditions for the accessibility and controllability of statistical linearization. Specifically, we establish simple sufficient algebraic conditions for the accessibility and controllability of statistical linearization, which involve the rank of the Lie algebra generated by the drift only. In addition, we show these latter algebraic conditions are essentially sharp, by means of a counterexample, and that they are generic with respect to the drift and the initial condition.

==> Others/TransversalityOldOld.tex <==
In this section, we provide some results which establish generic accessibility and controllability properties for \eqref{eq:syslin}. Specifically, we show that the various rank conditions involving the coupled dynamics $F$ which we listed in Section \ref{sec:AccConditions} hold \textit{generically} (in the sense of Thom's transversality) with respect to the drift $f$ and the diffusion $g$. In turn, due to Lemma \ref{lemma:Acc}--\ref{lemma:Contr}, these results enable generic accessibility and controllability of the linearized system \eqref{eq:syslin}.

From now we consider control-affine drift mappings uniquely, i.e.,
$$
f(x,u) = f_0(x) + \sum^m_{i=1} u_i f_i(x) ,
$$
and, by adopting the notation of Section \ref{sec:Main}, we define the vector fields
$$
\begin{aligned}
F_{f_0,g} : \quad &\mathbb{R}^n \times \Sym(n) \rightarrow \mathbb{R}^n \times \Sym(n) \\
&X = (m,P) \mapsto \vecdef{ f_0(m) }{ Df_0(m) P + P Df_0(m)^T + g(m) g(m)^{\top} } ,
\end{aligned}
$$
$$
\begin{aligned}
F_{f_i} : \quad &\mathbb{R}^n \times \Sym(n) \rightarrow \mathbb{R}^n \times \Sym(n) \\
&X = (m,P) \mapsto \vecdef{ f_i(m) }{ Df_i(m) P + P Df_i(m)^T } , \quad i=1,\dots,m .
\end{aligned}
$$
For every $\ell , r , s \in \mathbb{N}$, we introduce the following quantities (see, e.g., \cite{Hirsch1994}):
\begin{ItemizE}
    \item $\pi^{\ell}_{r,s} : J^{\ell}(\mathbb{R}^r;\mathbb{R}^s) \rightarrow \mathbb{R}^r$ is the vector bundle of $\ell$-jets of maps in $C^{\infty}(\mathbb{R}^r;\mathbb{R}^s)$;
    \item for every $h \in C^{\infty}(\mathbb{R}^r;\mathbb{R}^s)$, $j^{\ell}_{r,s}(h) : \mathbb{R}^r \rightarrow J^{\ell}(\mathbb{R}^r;\mathbb{R}^s)$ is the jet map associated with $\pi^{\ell}_{r,s}$; in particular, when clear from the context, for the sake of conciseness we denote $j^{\ell}(h)_y \in J^{\ell}(\mathbb{R}^r;\mathbb{R}^s)$, for every $h \in C^{\infty}(\mathbb{R}^r;\mathbb{R}^s)$ and every $y \in \mathbb{R}^r$.
\end{ItemizE}
We recall that the family of sets
$$
\Big\{ h \in C^{\infty}(\mathbb{R}^r;\mathbb{R}^s) : \ j^{\ell}(h)(\mathbb{R}^r) \subseteq U \Big\} , \ \textnormal{$U$ open subset of $J^{\ell}(\mathbb{R}^r;\mathbb{R}^s)$} ,
$$
generates the (weak) Whitney topology of $C^{\infty}(\mathbb{R}^r;\mathbb{R}^s)$.

\begin{theorem}[Accessibility with Respect to Generic Drift and Diffusion] \label{theo:Acc}
There exists an open and dense (with respect to (w.r.t.) the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}} \subseteq C^{\infty}(\mathbb{R}^n;\mathbb{R}^{n \times (m + 2)})$, such that for every $(f_0,f_1,\dots,f_m,g) \in \mathcal{O}_{\textnormal{Acc}}$, it holds
$$
\dim \textnormal{Lie}_X\Big\{ F_{f_0,g} , F_{f_1} , \dots , F_{f_m} \Big\} = n + \frac{n(n+1)}{2} , \ \textnormal{for every} \ X \in \mathbb{R}^n \times \textnormal{\Sym}(n)_{++} .
$$
\end{theorem}

\begin{theorem}[Accessibility with Respect to Generic Drift] \label{theo:Acc0}
There exists an open and dense (w.r.t. the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}_0} \subseteq C^{\infty}(\mathbb{R}^n;\mathbb{R}^{n \times (m + 1)})$, such that for every $(f_0,f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Acc}_0}$, it holds
$$
\dim \textnormal{Lie}_X\Big\{ F_{f_0,0} , F_{f_1} , \dots , F_{f_m} \Big\} = n + \frac{n(n+1)}{2} , \ \textnormal{for every} \ X \in \mathbb{R}^n \times \textnormal{\Sym}(n)_{++} .
$$
\end{theorem}

Together with Proposition \ref{prop:accCA}, Theorem \ref{theo:Acc0} readily yields the following corollary.

\begin{corollary}[Accessibility with Respect to Generic Drift] \label{coroll:Acc}
There exists an open and dense (w.r.t. the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}_0} \subseteq C^{\infty}(\mathbb{R}^n;\mathbb{R}^{n \times (m + 1)})$, such that for every $(f_0,f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Acc}_0}$ and every $g \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$, it holds
$$
\dim \textnormal{Lie}_X\Big\{ F_{f_0,g} , F_{f_1} , \dots , F_{f_m} \Big\} = n + \frac{n(n+1)}{2} , \ \textnormal{for every} \ X \in \Omega_g ,
$$
where $\Omega_g \subseteq \mathbb{R}^n \times \textnormal{\Sym}(n)_{++}$ is an open and dense subset which depends on $g$ uniquely.
\end{corollary}

\begin{theorem}[Controllability with Respect to Generic Drift] \label{theo:Contr}
Let $m \ge 2$. There exists an open and dense (with respect to the Whitney topology) subset $\mathcal{O}_{\textnormal{Contr}} \subseteq C^{\infty}(\mathbb{R}^n;\mathbb{R}^{n \times m})$, such that for every $(f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Contr}}$, it holds
$$
\dim \textnormal{Lie}_X\Big\{ F_{f_1} , \dots , F_{f_m} \Big\} = n + \frac{n(n+1)}{2} , \ \textnormal{for every} \ X \in \mathbb{R}^n \times \textnormal{\Sym}(n)_{++}  .
$$
\end{theorem}

\textcolor{red}{Riccardo: do we add any additional discussion on those theorems here?}

The rest of the section is devoted to the proof of these latter results. In particular, it suffices to prove Theorem \ref{theo:Acc} for $m = 1$ (the cases $m \ge 2$ result from the latter), given that the proofs of Theorem \ref{theo:Acc0} and Theorem \ref{theo:Contr} much follow the same line.

\subsection{Some concepts from algebraic geometry and transversality theory}

Before jumping into the proof of Theorem \ref{theo:Acc}, we recall some useful concepts from algebraic geometry and transversality theory which are key to achieve the aforementioned proof, for which we mainly refer to \cite{Whitney1957,Bochnak1998,Martinet1970}.

We start by introducing some useful concepts of algebraic geometry. Let $\ell , r \in \mathbb{N}$. A semi-algebraic set $\mathcal{SA} \subseteq \mathbb{R}^r$ is a subset of the form
\begin{equation} \label{eq:SemiAlg}
    \mathcal{SA} = \bigcup^{\ell}_{i = 1} \Big\{ y \in \mathbb{R}^r : \ p^i_1(y) = \dots = p^i_{a_i}(y) = 0 , \ q^i_1(y) < 0 , \dots , q^i_{b_i}(y) < 0 \Big\} ,
\end{equation}
for polynomials $p^i_j , q^i_j : \mathbb{R}^r \rightarrow \mathbb{R}$. Semi-algebraic sets enjoy the following properties:
\begin{ItemizE}
    \item finite unions of semi-algebraic sets are semi-algebraic sets;
    \item topological closures of semi-algebraic sets are semi-algebraic sets;
    \item projections of semi-algebraic sets are semi-algebraic sets; specifically, given $s \in \mathbb{N} \cap [1,r)$ and a semi-algebraic set $\mathcal{SA} \subseteq \mathbb{R}^r$, the following set is semi-algebraic:
    $$
    \Proj_{\mathbb{R}^s}(\mathcal{SA}) \subseteq \mathbb{R}^s , \quad \textnormal{where we denote} \quad \Proj_{\mathbb{R}^s}(y_1,\dots,y_r) = (y_1,\dots,y_s) .
    $$
\end{ItemizE}
A simple induction argument on \eqref{eq:SemiAlg} shows that semi-algebraic sets are disjoint unions of open subsets of algebraic sets. Thus, Whitney's stratification theorem readily yields the following representation result for semi-algebraic sets:

\begin{theorem}[Whitney's stratification for semi-algebraic sets] \label{theo:Whitney}
Let $r \in \mathbb{N}$ and $\mathcal{SA} \subseteq \mathbb{R}^r$ be a semi-algebraic set. There exist $\ell \in \mathbb{N}$ and embedded submanifolds $\mathcal{M}_1 , \dots , \mathcal{M}_{\ell} \subseteq \mathbb{R}^r$, which are mutually disjoint and such that
$$
\mathcal{SA} = \bigcup^{\ell}_{i = 1} \mathcal{M}_i \quad \textnormal{and} \quad \dim \mathcal{M}_{i+1} < \dim \mathcal{M}_i , \ i = 1 , \dots , \ell-1 .
$$
\end{theorem}

Thanks to Theorem \ref{theo:Whitney}, given $r \in \mathbb{N}$ and a semi-algebraic set $\mathcal{SA} \subseteq \mathbb{R}^r$, we may define the dimension and the codimension of $\mathcal{SA}$ as
$$
\dim \mathcal{SA} = \underset{i = 1,\dots,\ell}{\max} \dim \mathcal{M}_i \quad \textnormal{and} \quad \codim \mathcal{SA} = r - \dim \mathcal{SA} .
$$
Importantly, the topological closure does not modify the dimension, nor the codimension of a semi-algebraic set. Indeed, as a matter of example let $r \in \mathbb{N}$ and
$$
\mathcal{SA} = \big\{ y \in \mathbb{R}^r : \ p(y) = 0 , \ q(y) < 0 \big\} ,
$$
for polynomials $p , q : \mathbb{R}^r \rightarrow \mathbb{R}$. By definition, we must have
\begin{align*}
    \dim \overline{\mathcal{SA}} &\le \max \Big\{ \dim \mathcal{SA} \ , \ \dim \big\{ y \in \mathbb{R}^r : \ p(y) = q(y) = 0 \big\} \Big\} \\
    &\le \max \Big\{ \dim \mathcal{SA} \ , \ \dim \big\{ y \in \mathbb{R}^r : \ p(y) = 0 \big\} \Big\} = \dim \mathcal{SA} ,
\end{align*}
where we infer the last equality from the fact that $\mathcal{SA}$ is open in $p^{-1}(0)$, and thus
\begin{equation} \label{eq:DimClosure}
    \dim \overline{\mathcal{SA}} = \dim \mathcal{SA} \quad \textnormal{and} \quad \codim \overline{\mathcal{SA}} = \codim \mathcal{SA} .
\end{equation}
The extension of this property to general semi-algebraic sets follows by iterating the previous argument through classical induction.

Finally, for $s \in \mathbb{N} \cap [1,r)$ and a semi-algebraic set $\mathcal{SA} \subseteq \mathbb{R}^r$, a quick direct computation yields the following useful property of codimensions:
\begin{equation} \label{eq:DimProj}
    \codim \Proj_{\mathbb{R}^s}(\mathcal{SA}) \ge \codim \mathcal{SA} - (r - s) .
\end{equation}

We now turn to introducing some useful concepts of transversality theory. In what follows, for any given $\ell \in \mathbb{N}$, we consider the vector bundle of $\ell$-jets $J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$, for which we implicitly adopt the identification
\begin{equation} \label{eq:Identification}
    J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) \cong \mathbb{R}^{2 n + 3 n \sum^{\ell}_{i=1} {\scriptsize \left(\begin{array}{c}
    n + i - 1 \\
    i
\end{array}\right)}} ,
\end{equation}
through some (global) trivialization mapping. In particular, for every $f_0 , f_1 , g \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$ and every $m \in \mathbb{R}^n$, $j^{\ell}(f_0,f_1,g)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$ is identified to
\begin{align*}
j^{\ell}\big( f_0 , f_1 , g \big)_m = \bigg( m , \ &(\theta^{f_0}_0)^{1 \le k \le n} , (\theta^{f_1}_0)^{1 \le k \le n} , (\theta^g_0)^{1 \le k \le n} , \\
&(\theta^{f_0}_1)^{1 \le k \le n}_{0 \le i_1 \le n} , (\theta^{f_1}_1)^{1 \le k \le n}_{0 \le i_1 \le n} , (\theta^g_1)^{1 \le k \le n}_{0 \le i_1 \le n} , \\
&\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
&(\theta^{f_0}_{\ell})^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_{\ell} \le n} , (\theta^{f_1}_{\ell})^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_{\ell} \le n} , (\theta^g_{\ell})^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
where $(\theta^{f_0}_j)^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_j \le n} , (\theta^{f_1}_j)^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_j \le n} , (\theta^g_j)^{1 \le k \le n}_{0 \le i_1 \le \dots \le i_j \le n} \in \mathbb{R}^{n {\scriptsize \left(\begin{array}{c}
    n + j - 1 \\
    j
\end{array}\right)}}$.

\vspace{5pt}

From now on, we fix an integer $\ell \in \mathbb{N}$ (to be appropriately chosen later) and we introduce the product vector bundle
$$
\Pi_{\ell} : E_{\ell} = J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) \times_{\mathbb{R}^n} \mathbb{R} \times_{\mathbb{R}^n} \Sym(n) \rightarrow \mathbb{R}^n ,
$$
for which we implicitly adopt the identification
\begin{equation} \label{eq:Identification1}
    E_{\ell} \cong \mathbb{R}^{2 n + 1 + \frac{n(n+1)}{2} + 3 n \sum^{\ell}_{i=1} {\scriptsize \left(\begin{array}{c}
    n + i - 1 \\
    i
\end{array}\right)}} ,
\end{equation}
through some (global) trivialization mapping. In particular, with a slight abuse of notation, we denote the elements of $E_{\ell}$ by
$$
\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) = \big( j^{\ell}(f_0,f_1,g) , \alpha , P \big)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) \times_{\mathbb{R}^n} \mathbb{R} \times_{\mathbb{R}^n} \Sym(n) .
$$
Therefore, the projection
\begin{align*}
    \Proj_{J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})} : \ &E_{\ell} \rightarrow J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) \\
    &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \mapsto j^{\ell}(f_0,f_1,g)_m
\end{align*}
is a well-defined and smooth vector bundle homomorphism.

The identifications \eqref{eq:Identification} and \eqref{eq:Identification1} allow us to introduce semi-algebraic sets $\mathcal{SA} \subseteq J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$ and semi-algebraic sets $\mathcal{SA} \subseteq E_{\ell}$, and thus we can make use of the following key transversality result to prove Theorem \ref{theo:Acc}.

\begin{theorem}[Transversality Theorem for $E_{\ell}$] \label{theo:Transversality}
Let $\mathcal{SA} \subseteq J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$ be a closed semi-algebraic set which satisfies
$$
\codim \mathcal{SA} \ge n + 1 .
$$
Then, the subset
$$
\mathcal{O}_{\mathcal{SA}} = \Big\{ (f_0,f_1,g) \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^{3 n}) : \ j^{\ell}(f_0,f_1,g) \cap \mathcal{SA} = \emptyset \Big\}
$$
is open and dense (w.r.t. the Whitney topology) in $C^{\infty}(\mathbb{R}^n;\mathbb{R}^{3 n})$.
\end{theorem}

Theorem \ref{theo:Transversality} results from combining Theorem \ref{theo:Whitney} with the stratified version of Thom's transversality theorem (see \cite[Theorem 6.1 and ``Remarque'' at page 175]{Martinet1970}).

\subsection{Proof of Theorem \ref{theo:Acc}}

Our proof of Theorem \ref{theo:Acc} is inspired by the proofs in \cite{Lobry1972,Bonnard1997,Chitour2006}. We introduce appropriate, non-trivial modifications to these proofs to address singularities which are due to possibly trivial Lie brackets.

\subsubsection{Definition of the bad sets} Through a slight abuse of notation which is possible thanks to the identifications \eqref{eq:Identification} and \eqref{eq:Identification1}, for $r \in \mathbb{N} \cap [0,\ell]$ the mappings
$$
j^{\ell}(f_0,f_1,g)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) \mapsto \ad^r f_0 \cdot f_1(m) \in \mathbb{R}^n ,
$$
$$
\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} \mapsto \ad^r F_{f_0,g} \cdot F_{f_1}(X) \in \mathbb{R}^{n + \frac{n(n+1)}{2}} ,
$$
where $\ad^r$ is the $r$-iterated Lie bracket, are well-defined vector-valued polynomials. This remark, together with the identifications \eqref{eq:Identification} and \eqref{eq:Identification1}, allows us to defined the following \textit{bad sets}, which are semi-algebraic sets of $E_{\ell}$ and of $J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$, respectively:
\begin{align*}
    \mathcal{B}^{\ell}_1 = \bigg\{ &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 \neq 0 , \ \theta^{f_1}_0 \neq \alpha \theta^{f_0}_0 , \ \det P \neq 0 , \\
    & \rank \Big[ \ad \, F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell} F_{f_0,g} \cdot F_{f_1}(X) \Big] < n + \frac{n(n+1)}{2} \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^{\ell}_2 = \bigg\{ &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = \alpha \theta^{f_0}_0 , \ \alpha \neq 0 , \ \det P \neq 0 , \\
    & \rank \Big[ \ad \, F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell} F_{f_0,g} \cdot F_{f_1}(X) \Big] < n + \frac{n(n+1)}{2} \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^{\ell}_3 = \bigg\{ &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = 0 , \ \det P \neq 0 , \\
    &\hspace{29ex} \ad \, f_0 \cdot f_1(m) \neq 0 , \ \ad \, f_0 \cdot f_1(m) \neq \alpha \theta^{f_0}_0 , \\
    & \rank \Big[ \ad^2 F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell+1} F_{f_0,g} \cdot F_{f_1}(X) \Big] < n + \frac{n(n+1)}{2} \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^{\ell}_4 = \bigg\{ &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = 0 , \ \det P \neq 0 , \\
    &\hspace{29ex} \ad \, f_0 \cdot f_1(m) = \alpha \theta^{f_0}_0 , \ \alpha \neq 0 , \\
    & \rank \Big[ \ad^2 F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell+1} F_{f_0,g} \cdot F_{f_1}(X) \Big] < n + \frac{n(n+1)}{2} \bigg\} ,
\end{align*}
% \begin{align*}
%     \mathcal{B}^{\ell}_4 = \bigg\{ &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = 0 , \ \det P \neq 0 , \\
%     &\hspace{29ex} \ad \, f_0 \cdot f_1(m) = \alpha \theta^{f_0}_0 , \ \alpha \neq 0 \bigg\} ,
% \end{align*}
\begin{align*}
    \mathcal{B}^{\ell}_5 = \bigg\{ j^{\ell}(f_0,f_1,g)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n}) : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = \ad \, f_0 \cdot f_1(m) = 0 \bigg\} .
\end{align*}
Thanks to \eqref{eq:DimClosure} and \eqref{eq:DimProj}, we finally have that the \textit{bad set}
$$
\mathcal{B}^{\ell} = \overline{\Proj_{J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})}( \mathcal{B}^{\ell}_1\cup \mathcal{B}^{\ell}_2 \cup \mathcal{B}^{\ell}_3 \cup \mathcal{B}^{\ell}_4 ) \cup \mathcal{B}^{\ell}_5} \subseteq J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})
$$
is a semi-algebraic set whose codimension satisfies
\begin{equation} \label{eq:TestCodim}
    \codim \mathcal{B}^{\ell} \ge \max \left\{ \underset{i=1,\dots,4}{\max} \left\{ \codim \mathcal{B}^{\ell}_i - \left( \frac{n(n+1)}{2} + 1 \right) \right\} , \codim \mathcal{B}^{\ell}_5 \right\} .
\end{equation}

\subsubsection{Existence of an open and dense subset}

Assume that
\begin{equation} \label{eq:ReqCodim}
    \codim \mathcal{B}^{\ell}_i \ge \frac{n(n+1)}{2} + n + 2 , \quad i = 1,\dots,5 , \quad \textnormal{for some} \ \ell \in \mathbb{N} .
\end{equation}
Therefore, \eqref{eq:TestCodim} yields $\codim \mathcal{B}^{\ell} \ge n + 1$ and we can apply Theorem \ref{theo:Transversality} to infer the existence of an open and dense (with respect to the Whitney topology) subset
$$
\mathcal{O}_{\textnormal{Acc}} = \Big\{ (f_0,f_1,g) \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^{3 n}) : \ j^{\ell}(f_0,f_1,g) \cap \mathcal{B}^{\ell} = \emptyset \Big\} \subseteq C^{\infty}(\mathbb{R}^n;\mathbb{R}^{3 n}) .
$$
In particular, straightforward computations by contradiction show that
$$
(f_0,f_1,g) \in \mathcal{O}_{\textnormal{Acc}} \ \Longrightarrow \ \dim \textnormal{Lie}_X\Big\{ F_{f_0,g} , F_{f_1} \Big\} = n + \frac{n(n+1)}{2} , \ \textnormal{if} \ f_0(m) , \det P \neq 0 .
$$
At this step, since the algebraic set of $\ell$-jets $j^{\ell}(f_0,f_1,g)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{3 n})$ which satisfy $\theta^{f_0}_0 = \theta^{f_0}_1 = 0$ has codimension $2 n$ (see, e.g., \cite{Lobry1972}), up to swapping $f_0$ and $f_1$ in the definition of the bad sets $\mathcal{B}^{\ell}_1 , \dots , \mathcal{B}^{\ell}_5$, one easily concludes that the proof of Theorem \ref{theo:Acc} is achieved once \eqref{eq:ReqCodim} is proved to hold true.

\subsubsection{Codimension computations}

The rest of the manuscript is devoted to prove \eqref{eq:ReqCodim}. We provide computations for $\mathcal{B}^{\ell}_2$ and $\mathcal{B}^{\ell}_4$ uniquely, given that these latter boil down to the most challenging non-trivial steps, whereas the computations for $\mathcal{B}^{\ell}_1$, $\mathcal{B}^{\ell}_3$, and $\mathcal{B}^{\ell}_5$ are simpler and essentially follow the same line.

In what follows, we fix any $\ell \ge n + \frac{n(n+1)}{2}$ (to be selected later), and for $r \in \mathbb{N} \cap [1,\ell]$ and $h , h_1 , \dots , h_r \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$, we denote the matrix-valued mapping
$$
\big( (D^{r+1} h) h_1 \dots h_r \big)_{i j}(m) = \sum^n_{i_1,\dots,i_r=1} \frac{\partial^{r+1} h^i}{\partial x^j \partial x^{i_1} \dots \partial x^{i_r}}(m) fh^{i_1}_1(m) \dots h^{i_r}_r(m) \in \mathbb{R}^{n \times n} .
$$
Also, we denote the symmetric tensorization of any element $\theta_r \in \mathbb{R}^{n {\scriptsize \left(\begin{array}{c}
    n + r - 1 \\
    r
\end{array}\right)}}$ by
$$
S(\theta_r) : \underbrace{\mathbb{R}^n \times \dots \times \mathbb{R}^n}_{r-\textnormal{times}} \rightarrow \mathbb{R}^n ,
$$
whereas denote the symmetrization of a matrix $A \in \mathbb{R}^n$ by $\Sym(A) = A + A^{\top}$. For every $\rho \in [0,\ell]$, we denote by $L^{\rho}_{n,\ell}$ the Stiefel manifold of linear mappings
$$
L : \mathbb{R}^{\ell} \rightarrow \mathbb{R}^{n + \frac{n(n+1)}{2}}
$$
such that $\rank L = \rho$, for which
\begin{equation} \label{eq:Stiefel}
    \codim L^{\rho}_{n,\ell} = \left( n + \frac{n(n+1)}{2} - \rho \right) (\ell - \rho) .
\end{equation}
Finally, we introduce symbols such as $A(\neq a)$ to denote a general polynomial expression $A$ which does not depend on the general variable $a$.

\vspace{5pt}

\textbf{Computations for $\bm{\mathcal{B}^{\ell}_2}$.}

\vspace{5pt}

Straightforward, though lengthy computations by induction yield the following:

\begin{lemma} \label{lemma:FirstBrackets}
For every $r \in \mathbb{N}$ and every $f_0, f_1 , g \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$, it holds:
\begin{align*}
    \ad^r F_{f_0,g} \cdot F_{f_1}(X) = &\left(\begin{array}{c}
        A_{r}\big( \neq D^{i+1} f_0 , D^i f_1 , i \ge r \big) \\[10pt]
        B_{r}\big( \neq D^i f_0 , D^{i+1} f_1 , i \ge r+1 \big)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        (D^r f_1) \underbrace{f_0 \dots f_0}_{r-\textnormal{times}} \\
        -\textnormal{\Sym}\Big( (D^{r+1} f_0) f_1 \underbrace{f_0 \dots f_0}_{(r-1)-\textnormal{times}} P \Big)
    \end{array}\right) ,
\end{align*}
for polynomial expressions $A_r$ and $B_r$ of the derivatives of $f_0$, $f_1$, and $g$.
\end{lemma}

At this step, let us introduce the subset
$$
\mathcal{S}^2_{\ell} = \Big\{ \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_0 = \alpha \theta^{f_0}_0 , \ \alpha \neq 0 , \ \det P \neq 0 \Big\} .
$$
Since the mapping
\begin{align*}
    \mathcal{F}^2_{\ell} : \ &E_{\ell} \rightarrow \mathbb{R}^n \\
    &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \mapsto \theta^{f_1}_0 - \alpha \theta^{f_0}_0
\end{align*}
is a submersion, we infer that
$$
\mathcal{S}^2_{\ell} = ( \mathcal{F}^2_{\ell} )^{-1}(0) \setminus \Big\{ \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 = 0 \ \textnormal{or} \ \alpha = 0 \ \textnormal{or} \ \det P = 0 \Big\}
$$
is an embedded submanifold of $E_{\ell}$ with $\dim \mathcal{S}^2_{\ell} = \dim E_{\ell} - n$, and which contains $\mathcal{B}^2_{\ell}$. Since for a fixed $q = \big( j^{\ell}(\tilde f_0,\tilde f_1,\tilde g)_m , \tilde \alpha , \tilde P \big) \in \mathcal{B}^2_{\ell}$ it holds that $\theta^{\tilde f_0}_0 \neq 0$, we may select constant vectors $v_2 , \dots , v_n \in \mathbb{R}^n$ such that
$$
\{ v_1(p) , v_2(p) , \dots , v_n(p) \} = \{ \theta^{f_0}_0 , v_2 , \dots , v_n \} , \quad p = \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{U}_q
$$
spans $\mathbb{R}^n$ in an open neighborhood $\mathcal{U}_q \subseteq E_{\ell}$ of $q$. Therefore, the smooth mapping
\begin{align*}
    \psi\Big( &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \Big) = \bigg( m , \alpha , P , (\theta^{f_0}_0)^{1 \le k \le n} , \\
    &(\theta^{f_1}_0)^{1 \le k \le n} - \alpha (\theta^{f_0}_0)^{1 \le k \le n} , (\theta^g_0)^{1 \le k \le n} , \\
    &\psi^{f_0}_1 = \Big( S(\theta^{f_0}_1) v_{i_1} \Big)_{1 \le i_1 \le n} , \psi^{f_1}_1 = \Big( S(\theta^{f_1}_1) v_{i_1} \Big)_{1 \le i_1 \le n} ,  (\theta^g_1)^{1 \le k \le n}_{1 \le i_1 \le n} , \\
    &\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
    &\Big( \psi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(\theta^{f_0}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , \\
    &\Big( \psi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(\theta^{f_1}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , (\theta^g_{\ell})^{1 \le k \le n}_{1 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
which is defined in $\mathcal{U}_q$, is a local chart for $E_{\ell}$ which is in addition adapted to $\mathcal{S}^2_{\ell}$ at $q$.

For every $\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{S}^2_{\ell} \cap \mathcal{U}_q$, let $M = M(\theta^{f_0}_0,P)$ denote the matrix which corresponds to the smooth change of coordinates
$$
P^j = \sum^n_{i=1} M_{ij}(\theta^{f_0}_0,P) v_i , \quad M(\theta^{f_0}_0,P) = \big( M_{ij}(\theta^{f_0}_0,P) \big)_{1 \le i , j \le n} ,
$$
where $P^j$ denotes the $j$th column of $P$. Thus, for $r \in \mathbb{N}$ we may compute
\begin{align*}
    (D^{r+1} f_0) &f_1 \underbrace{f_0 \dots f_0}_{(r-1)-\textnormal{times}} P = \alpha \left( S(\theta^{f_0}_{r+1}) \underbrace{\theta^{f_0}_0 \dots \theta^{f_0}_0}_{r-\textnormal{times}} P^1 \Big| \ \dots \ \Big| S(\theta^{f_0}_{r+1}) \underbrace{\theta^{f_0}_0 \dots \theta^{f_0}_0}_{r-\textnormal{times}} P^n \right) \\[10pt]
    &= \left( S(\theta^{f_0}_{r+1}) v_1 \dots v_1 v_1 \Big| S(\theta^{f_0}_{r+1}) v_1 \dots v_1 v_2 \Big| \ \dots \ \Big| S(\theta^{f_0}_{r+1}) v_1 \dots v_1 v_n \right) (\alpha M) \\[10pt]
    &= \Big( \psi^{f_0}_{r+1;\{1,\dots,1,1\}} \Big| \psi^{f_0}_{r+1;\{1,\dots,1,2\}} \Big| \ \dots \ \Big| \psi^{f_0}_{r+1;\{1,\dots,1,n\}} \Big) (\alpha M) ,
\end{align*}
which together with Lemma \ref{lemma:FirstBrackets} finally yields
\begin{align} \label{eq:TransformedBracket}
    &\ad^r F_{f_0,g} \cdot F_{f_1}(X) = \left(\begin{array}{c}
        A_r\big( \neq \psi^{f_0}_{i+1} , \psi^{f_1}_i , i \ge r \big) \\[10pt]
        B_r\big( \neq \psi^{f_0}_i , \psi^{f_1}_{i+1} , i \ge r+1 \big)
    \end{array}\right) + \\[10pt]
    &+ \left(\begin{array}{c}
        \psi^{f_1}_{r;\{1,\dots,1\}} \\[10pt]
        -\textnormal{Sym}\bigg( \Big( \psi^{f_0}_{r+1;\{1,\dots,1,1\}} \big| \psi^{f_0}_{r+1;\{1,\dots,1,2\}} \big| \ \dots \ \big| \psi^{f_0}_{r+1;\{1,\dots,1,n\}} \Big) (\alpha M) \bigg)
    \end{array}\right) . \nonumber
\end{align}
for every $\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{S}^2_{\ell} \cap \mathcal{U}_q$ and every $r \in \mathbb{N} \cap [1,\ell]$.

At this step, up to appropriate identifications, the triangular form of \eqref{eq:TransformedBracket} allows us to infer that, for every $\ell \ge n + \frac{n(n+1)}{2}$, the mappings
$$
\mathcal{L}^{\ell}_q = \Big[ \ad \, F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell} F_{f_0,g} \cdot F_{f_1}(X) \Big] : \ \mathcal{S}^2_{\ell} \cap \mathcal{U}_q \rightarrow \mathbb{R}^{\left( n + \frac{n(n+1)}{2} \right) \times \ell}
$$
are \textcolor{red}{submersions (Riccardo: that is wrong! The columns of this matrices are not linearly independent...)}, and therefore $(\mathcal{L}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) \subseteq \mathcal{S}^2_{\ell} \cap \mathcal{U}_q$ are submanifolds for every $\rho \in [0,\ell]$, which due to \eqref{eq:Stiefel} satisfy
\begin{equation} \label{eq:Stiefel1}
    \codim (\mathcal{L}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) = \codim L^{\rho}_{n,\ell} = \left( n + \frac{n(n+1)}{2} - \rho \right) ( \ell - \rho ) .
\end{equation}
Since
$$
\mathcal{B}^{\ell}_2 \cap \mathcal{U}_q \subseteq \bigcup^{n + \frac{n(n+1)}{2} - 1}_{\rho = 1} (\mathcal{L}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) ,
$$
thanks to \eqref{eq:Stiefel1} we finally obtain that
\begin{align*}
    \codim \mathcal{B}^{\ell}_2 \cap \mathcal{V}_q &\ge \codim (\mathcal{L}^{\ell}_q)^{-1}\left( L^{n + \frac{n(n+1)}{2} - 1}_{n,\ell} \right) \\
    &= \ell - n - \frac{n(n+1)}{2} + 1 \ge \frac{n(n+1)}{2} + n + 2 ,
\end{align*}
as soon as we select $\ell \ge n^2 + 3 n + 1$. The arbitrariness of $q \in \mathcal{B}^{\ell}_2$ allows us to conclude that \eqref{eq:ReqCodim} holds true for $\mathcal{B}^2_{\ell}$ with $\ell \ge n^2 + 3 n + 1$.

\vspace{5pt}

\textbf{Computations for $\bm{\mathcal{B}^{\ell}_4}$.}

\vspace{5pt}

In this case, linear independence between the vector field $f_0$ and the Lie bracket $\ad \, f_0 \cdot f_1$ is lost, yielding singularities which turn the differential of \eqref{eq:TransformedBracket} into a non-surjective mapping. Thus, the result of Lemma \ref{lemma:FirstBrackets} must be appropriately modified, and in particular additional lengthy computations by induction yield the following:

\begin{lemma} \label{lemma:SecondBrackets}
For every $r \in \mathbb{N}$, $r \ge 2$ and every $f_0, f_1 , g \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$, it holds:
\begin{align*}
    &\ad^r F_{f_0,g} \cdot F_{f_1}(X) = \left(\begin{array}{c}
        C_{r}\big( \neq D^i f_0 , D^i f_1 , i \ge r \big) \\[10pt]
        D_{r}\big( \neq D^i f_0 , D^{i+2} f_1 , i \ge r \big)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        (D^r f_1) \underbrace{f_0 \dots f_0}_{r-\textnormal{times}} \\
        \textnormal{\Sym}\Big( \big( -3 (D^r f_0) \ad \, f_0 \cdot f_1 + (D f_1) (D^r f_0) f_0 \big) \underbrace{f_0 \dots f_0}_{(r-2)-\textnormal{times}} P \Big)
    \end{array}\right) , \ \textnormal{if} \ f_1(m) = 0 ,
\end{align*}
for polynomial expressions $C_r$ and $D_r$ of the derivatives of $f_0$, $f_1$, and $g$.
\end{lemma}

At this step, let us introduce the subset
\begin{align*}
    \mathcal{S}^4_{\ell} = \Big\{ \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ &\theta^{f_0}_0 \neq 0 , \ \theta^{f_1}_1 \theta^{f_0}_0 = \alpha \theta^{f_0}_0 , \ \alpha \neq 0 , \\
    & \det P \neq 0 , \ \det\big( \theta^{f_1}_1 - 3 \alpha I \big) \neq 0 \Big\} .
\end{align*}
Since the mapping
\begin{align*}
    \mathcal{F}^4_{\ell} : \ &E_{\ell} \setminus \Big\{ \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ \theta^{f_0}_0 = 0 \Big\} \rightarrow \mathbb{R}^n \\
    &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \mapsto \theta^{f_1}_1 \theta^{f_0}_0 - \alpha \theta^{f_0}_0
\end{align*}
is a submersion, we infer that
\begin{align*}
    \mathcal{S}^4_{\ell} = ( \mathcal{F}^4_{\ell} )^{-1}(0) \setminus \Big\{ \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in E_{\ell} : \ &\alpha = 0 \ \textnormal{or} \ \det P = 0 \\
    & \textnormal{or} \ \det\big( \theta^{f_1}_1 - 3 \alpha I \big) = 0 \Big\}
\end{align*}
is an embedded submanifold of $E_{\ell}$ with $\dim \mathcal{S}^4_{\ell} = \dim E_{\ell} - n$, and which contains $\mathcal{B}^4_{\ell}$. Since for a fixed $q = \big( j^{\ell}(\tilde f_0,\tilde f_1,\tilde g)_m , \tilde \alpha , \tilde P \big) \in \mathcal{B}^4_{\ell}$ it holds that $\theta^{\tilde f_0}_0 \neq 0$, let $v_2 , \dots , v_n \in \mathbb{R}^n$ be the previously introduced constant vectors such that
$$
\{ v_1(p) , v_2(p) , \dots , v_n(p) \} = \{ \theta^{f_0}_0 , v_2 , \dots , v_n \} , \quad p = \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{U}_q
$$
spans $\mathbb{R}^n$ in the open neighborhood $\mathcal{U}_q \subseteq E_{\ell}$ of $q$. Therefore, the smooth mapping
\begin{align*}
    \phi\Big( &\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \Big) = \bigg( m , \alpha , P , (\theta^{f_0}_0)^{1 \le k \le n} , (\theta^{f_1}_0)^{1 \le k \le n} , (\theta^g_0)^{1 \le k \le n} , \\
    &(\theta^{f_0}_1)^{1 \le k \le n}_{1 \le i_1 \le n} \\
    &\phi^{f_1}_1 = \Big( S(\theta^{f_1}_1) v_1 - \alpha v_1 \ \Big| \ S(\theta^{f_1}_1) v_2 \ \Big| \ \dots \ \Big| \ S(\theta^{f_1}_1) v_n \Big) , (\theta^g_1)^{1 \le k \le n}_{1 \le i_1 \le n} , \\
    &\Big( \phi^{f_0}_{\ell;\{i_1,i_2\}} \Big)_{1 \le i_1 \le i_2 \le n} = \Big( S(\theta^{f_0}_2) v_{i_1} v_{i_2} \Big)_{1 \le i_1 \le i_2 \le n} , \\
    &\Big( \phi^{f_1}_{\ell;\{i_1,i_2\}} \Big)_{1 \le i_1 \le i_2 \le n} = \Big( S(\theta^{f_1}_2) v_{i_1} v_{i_2} \Big)_{1 \le i_1 \le i_2 \le n} ,  (\theta^g_2)^{1 \le k \le n}_{1 \le i_1 \le i_2 \le n} , \\
    &\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
    &\Big( \phi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(\theta^{f_0}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , \\
    &\Big( \phi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(\theta^{f_1}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , (\theta^g_{\ell})^{1 \le k \le n}_{1 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
which is defined in $\mathcal{U}_q$, is a local chart for $E_{\ell}$ which is in addition adapted to $\mathcal{S}^4_{\ell}$ at $q$.

For every $\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{S}^4_{\ell} \cap \mathcal{U}_q$, let $N = N(\theta^{f_0}_0,P)$ denote the matrix which corresponds to the smooth change of coordinates
$$
P^j = \sum^n_{i=1} N_{ij}(\theta^{f_0}_0,P) v_i , \quad N(\theta^{f_0}_0,P) = \big( N_{ij}(\theta^{f_0}_0,P) \big)_{1 \le i , j \le n} ,
$$
where $P^j$ denotes the $j$th column of $P$. Thus, for $r \in \mathbb{N}$, $r \ge 2$ we may compute
\begin{align} \label{eq:TransformationOfBrackets}
    \big( -3 &\ (D^r f_0) \ad \, f_0 \cdot f_1 + (D f_1) (D^r f_0) f_0 \big) \underbrace{f_0 \dots f_0}_{(r-2)-\textnormal{times}} P = \\
    &= \left( ( \theta^{f_1}_1 - 3 \alpha I ) S(\theta^{f_0}_r) \underbrace{\theta^{f_0}_0 \dots \theta^{f_0}_0}_{(r-1)-\textnormal{times}} P^1 \Big| \ \dots \ \Big| ( \theta^{f_1}_1 - 3 \alpha I ) S(\theta^{f_0}_r) \underbrace{\theta^{f_0}_0 \dots \theta^{f_0}_0}_{(r-1)-\textnormal{times}} P^n \right) \nonumber \\[10pt]
    &= ( \theta^{f_1}_1 - 3 \alpha I ) \left( S(\theta^{f_0}_r) v_1 \dots v_1 v_1 \Big| S(\theta^{f_0}_r) v_1 \dots v_1 v_2 \Big| \ \dots \ \Big| S(\theta^{f_0}_r) v_1 \dots v_1 v_n \right) N \nonumber \\[10pt]
    &= \mathcal{G}(\alpha,\phi^{f_0}_0,\phi^{f_1}_1) \Big( \phi^{f_0}_{r;\{1,\dots,1,1\}} \Big| \phi^{f_0}_{r;\{1,\dots,1,2\}} \Big| \ \dots \ \Big| \phi^{f_0}_{r;\{1,\dots,1,n\}} \Big) N , \nonumber
\end{align}
where
$$
\mathcal{G} : \mathcal{S}^4_{\ell} \cap \mathcal{U}_q \rightarrow \mathbb{R}^{n \times n}
$$
is a smooth mapping which depends on $\alpha$, $\phi^{f_0}_0$, and $\phi^{f_1}_1$ uniquely. Note that
\begin{equation} \label{eq:det}
    \det \mathcal{G}(\alpha,\phi^{f_0}_0,\phi^{f_1}_1) \neq 0 , \quad \textnormal{for every} \quad \big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{S}^4_{\ell} \cap \mathcal{U}_q .
\end{equation}
Finally, together with Lemma \ref{lemma:FirstBrackets}, \eqref{eq:TransformationOfBrackets} finally yields
\begin{align} \label{eq:TransformedBracket}
    &\ad^r F_{f_0,g} \cdot F_{f_1}(X) = \left(\begin{array}{c}
        C_r\big( \neq \phi^{f_0}_i , \phi^{f_1}_i , i \ge r \big) \\[10pt]
        D_r\big( \neq \phi^{f_0}_i , \phi^{f_1}_{i+2} , i \ge r \big)
    \end{array}\right) + \\[10pt]
    &+ \left(\begin{array}{c}
        \phi^{f_1}_{r;\{1,\dots,1\}} \\[10pt]
        \textnormal{Sym}\bigg( \mathcal{G}(\alpha,\phi^{f_0}_0,\phi^{f_1}_1) \Big( \phi^{f_0}_{r;\{1,\dots,1,1\}} \Big| \phi^{f_0}_{r;\{1,\dots,1,2\}} \Big| \ \dots \ \Big| \phi^{f_0}_{r;\{1,\dots,1,n\}} \Big) N \bigg)
    \end{array}\right) . \nonumber
\end{align}
for every $\big( j^{\ell}(f_0,f_1,g)_m , \alpha , P \big) \in \mathcal{S}^4_{\ell} \cap \mathcal{U}_q$ and every $r \in \mathbb{N} \cap [2,\ell]$.

At this step, up to appropriate identifications, \eqref{eq:det} and the triangular form of \eqref{eq:TransformedBracket} allow us to infer that, for every $\ell \ge n + \frac{n(n+1)}{2}$, the mappings
$$
\mathcal{H}^{\ell}_q = \Big[ \ad \, F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell} F_{f_0,g} \cdot F_{f_1}(X) \Big] : \ \mathcal{S}^4_{\ell} \cap \mathcal{U}_q \rightarrow \mathbb{R}^{\left( n + \frac{n(n+1)}{2} \right) \times \ell}
$$
are submersions, and therefore $(\mathcal{H}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) \subseteq \mathcal{S}^4_{\ell} \cap \mathcal{U}_q$ are submanifolds for every $\rho \in [0,\ell]$, which due to \eqref{eq:Stiefel} satisfy
\begin{equation} \label{eq:Stiefel1}
    \codim (\mathcal{H}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) = \codim L^{\rho}_{n,\ell} = \left( n + \frac{n(n+1)}{2} - \rho \right) ( \ell - \rho ) .
\end{equation}
Since
$$
\mathcal{B}^{\ell}_2 \cap \mathcal{U}_q \subseteq \bigcup^{n + \frac{n(n+1)}{2} - 1}_{\rho = 1} (\mathcal{L}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) ,
$$
thanks to \eqref{eq:Stiefel1} we finally obtain that
\begin{align*}
    \codim \mathcal{B}^{\ell}_2 \cap \mathcal{V}_q &\ge \codim (\mathcal{L}^{\ell}_q)^{-1}\left( L^{n + \frac{n(n+1)}{2} - 1}_{n,\ell} \right) \\
    &= \ell - n - \frac{n(n+1)}{2} + 1 \ge \frac{n(n+1)}{2} + n + 2 ,
\end{align*}
as soon as we select $\ell \ge n^2 + 3 n + 1$. The arbitrariness of $q \in \mathcal{B}^{\ell}_2$ allows us to conclude that \eqref{eq:ReqCodim} holds true for $\mathcal{B}^2_{\ell}$ with $\ell \ge n^2 + 3 n + 1$.

==> Preliminaries.tex <==
Consider a dynamics described by a stochastic differential equation of the form
\begin{equation} \label{eq:eds}
dx_t  = f(x_t,u) dt + \G(x_t)dW_t
\end{equation}
where $x_t \in \R^n$ is the state, $u \in \R^k$ the control, $W_t \in \R^p$ a Wiener process. Such equations are frequently used to model controlled systems with uncertainties or subject to random perturbations. However, there remain challenges in dealing with stochastic systems, in particular when performing optimal control. Indeed, stochastic optimal control methods are generally less numerically efficient than deterministic ones, and struggle to solve large-scale problems. An answer to that issue is to approximate the solution of the stochastic problem using the deterministic optimal control framework. Our approach works as follows. We assume that the cost of the optimal control problem is formulated as a quadratic function of both state and control; therefore all the data of the problem only depend on the first two moments of $x_t$. This allows us to use a statistical linearization method in order to approximate the mean and the covariance of $x_t$ as $(m,P)$ solution of the following system of ordinary differential equations 
\begin{equation} \label{eq:syslin}
\begin{cases}
\dot{m}(t) &= f(m(t),u(t))\\
\dot{P}(t) &= D_xf(m(t),u(t)) P(t) + P(t) D_xf(m(t),u(t))^T + g(m(t))g(m(t))^T. \\
\end{cases}
\end{equation}
The accuracy of this approximation is proven in ... Thus, the single objective of optimally controlling the mean trajectory of $x_t$ could be achieved by solving a deterministic optimal control problem on $m$. However, this will not insure the robustness of the solution, since the sample trajectories will be dispersed around the mean trajectory. Robustness would be guaranteed only if the dispersion stays small along the trajectory, which corresponds to minimizing the norm of $P$. Consequently, approximating the optimal control of \eqref{eq:eds} thanks to statistical linearization requires to have control on both variables $m$ and $P$ of the system \eqref{eq:syslin}.

==> TransversalityOld.tex <==
In this section, we conclude our study by establishing generic accessibility and controllability properties for \eqref{eq:syslin}. Specifically, we show that the various rank conditions involving the coupled dynamics \eqref{eq:vf_statlin} which we listed in Section \ref{sec:AccConditions} hold \textit{generically} (in the sense of Thom's transversality) with respect to the drift $f$. In turn, due to Lemma \ref{lemma:Acc}--\ref{lemma:Contr}, these results enable generic accessibility and controllability for the linearized system \eqref{eq:syslin}.

From now on, we consider control-affine drift mappings uniquely, i.e.,
$$
f(x,u) = f_0(x) + \sum^{\ncontrol}_{i=1} u_i f_i(x) , \quad u \in \U=\R^{\ncontrol} ,
$$
% and, by adopting the notation of Section \ref{sec:Main}, we define the vector fields
% $$
% \begin{aligned}
% F_{f_0,g} : \quad &\mathbb{R}^n \times \Sym(n) \rightarrow \mathbb{R}^n \times \Sym(n) \\
% &X = (m,P) \mapsto \vecdef{ f_0(m) }{ Df_0(m) P + P Df_0(m)^T + g(m) g(m)^{\top} } ,
% \end{aligned}
% $$
% $$
% \begin{aligned}
% F_{f_i} : \quad &\mathbb{R}^n \times \Sym(n) \rightarrow \mathbb{R}^n \times \Sym(n) \\
% &X = (m,P) \mapsto \vecdef{ f_i(m) }{ Df_i(m) P + P Df_i(m)^T } , \quad i=1,\dots,\ncontrol .
% \end{aligned}
% $$
and we thus adopt the notation we introduced through \eqref{eq:sysca}. For an open subset $\M$ of $\R^n$ and $\ell , r \in \mathbb{N}$, we introduce the following quantities (see, e.g., \cite{Hirsch1994}):
\begin{ItemizE}
    \item $\pi^{\ell}_r : J^{\ell}(\M;\mathbb{R}^r) \rightarrow \M$ is the vector bundle of $\ell$-jets of maps in $C^{\infty}(\M;\mathbb{R}^r)$;
    \item for every $h \in C^{\infty}(\M;\mathbb{R}^r)$, $j^{\ell}_r(h) : \M \rightarrow J^{\ell}(\M;\mathbb{R}^r)$ is the jet map associated with $\pi^{\ell}_r$; in particular, when clear from the context, for the sake of conciseness we denote $j^{\ell}(h)_y = j^{\ell}(h)(y) \in J^{\ell}(\M;\mathbb{R}^r)$, for every $h \in C^{\infty}(\M;\mathbb{R}^r)$ and every $y \in \M$.
\end{ItemizE}
We recall that the family of sets
$$
\Big\{ h \in C^{\infty}(\M;\mathbb{R}^r) : \ j^{\ell}(h)(\M) \subset \mathcal{V} \Big\} , \quad \textnormal{$\mathcal{V}$ open subset of $J^{\ell}(\M;\mathbb{R}^r)$} ,
$$
generates the (weak) Whitney topology of $C^{\infty}(\M;\mathbb{R}^r)$. Our main results are as follows.

% Riccardo: not sure this result holds true.
% \begin{theorem}[Accessibility with Respect to Generic Drift and Diffusion] \label{theo:Acc0}
% There exists an open and dense (with respect to (w.r.t.) the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}_0} \subset C^{\infty}(\mathbb{R}^n;\mathbb{R}^{n \times (m + 2)})$, such that for every $(f_0,f_1,\dots,f_m,g) \in \mathcal{O}_{\textnormal{Acc}_0}$, it holds
% \begin{align*}
%     \dim \textnormal{Lie}_X\Big\{ F_{f_i} , \ \ad^r F_{f_0,g} \cdot F_{f_i} : \ r \in \mathbb{N} \cap (0,\infty) , \ &i = 1,\dots,m \Big\} = N , \\
%     &\textnormal{for every} \ X \in \mathbb{R}^n \times \Sym(n)^{++} .
% \end{align*}
% \end{theorem}

\begin{theorem}[Weak Accessibility with Respect to Generic Drift] \label{theo:Acc}
There exists an open and dense (w.r.t. the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}} \subset C^{\infty}(\M;\mathbb{R}^{n \times (m + 1)})$, such that for every $(f_0,f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Acc}}$, it holds
$$
\dim \lie_{(m,P)} (\F_{0}) = N , \quad \textnormal{for every} \ (m,P) \in \M \times \Sym^+(n) ,
$$
where $\F_{0}$ is the family of vector fields \eqref{eq:vf_statlin}, which is generated by $F_{f_0,0} , F_{f_1} , \dots , F_{f_m}$.
% \begin{align*}
%     %\dim \textnormal{Lie}_X\Big\{ F_{f_i} , \ \ad^r F_{f_0,0} \cdot F_{f_i} : \ r \in \mathbb{N} \cap (0,\infty) , \ &i = 1,\dots,m \Big\} = N , \\
%     \dim \textnormal{Lie}_X\Big\{ F_{f_0,0} , \ F_{f_i} : \ i = 1,\dots,m \Big\} = \ &N \\
%     &\textnormal{for every} \ X \in \mathbb{R}^n \times \Sym(n)^{++} .
% \end{align*}
\end{theorem}

Theorem \ref{theo:Acc} may be refined as in the following result:

\begin{theorem}[Strong Accessibility with Respect to Generic Drift] \label{theo:Acc+}
There exists an open and dense (w.r.t. the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}_+} \subset C^{\infty}(\M;\mathbb{R}^{n \times (m + 1)})$, such that for every $(f_0,f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Acc}_+}$, it holds
$$
\dim \I_{(m,P)} (\F_{0}) = N , \quad \textnormal{for every} \ (m,P) \in \M \times \Sym^+(n) ,
$$
where $\F_{0}$ is the family of vector fields \eqref{eq:vf_statlin}, which is generated by $F_{f_0,0} , F_{f_1} , \dots , F_{f_m}$.
% \begin{align*}
%     \dim \textnormal{Lie}_X\Big\{ F_{f_i} , \ \ad^r F_{f_0,0} \cdot F_{f_i} : \ r \in \mathbb{N} \cap (0,\infty) , \ &i = 1,\dots,m \Big\} = N , \\
%     %\dim \textnormal{Lie}_X\Big\{ F_{f_0,0} , \ F_{f_i} : \ i = 1,\dots,m \Big\} = \ &N \\
%     &\textnormal{for every} \ X \in \mathbb{R}^n \times \Sym(n)^{++} .
% \end{align*}
\end{theorem}

Together with Proposition \ref{prop:accCA}, Theorem \ref{theo:Acc+} readily yields the following corollary.

\begin{corollary}[Accessibility with Respect to Generic Drift and Initial Datum] \label{coroll:AccTotal}
There exists an open and dense (w.r.t. the Whitney topology) subset $\mathcal{O}_{\textnormal{Acc}_+} \subset C^{\infty}(\M;\mathbb{R}^{n \times (m + 1)})$, such that for every $(f_0,f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Acc}_+}$ and every smooth diffusion mapping $g \in C^{\infty}(\M;\mathbb{R}^n)$, it holds
$$
\dim \I_{(m,P)} (\F_g) = N , \quad \textnormal{for every} \ (m,P) \in \Omega_g ,
$$
% \begin{align*}
%     \dim \textnormal{Lie}_X\Big\{ F_{f_i} , \ \ad^r F_{f_0,g} \cdot F_{f_i} : \ r \in \mathbb{N} \cap (0,\infty) , \ i = 1,\dots,m \Big\} = \  &N , \\
%     %\dim \textnormal{Lie}_X\Big\{ F_{f_0,g} , \ F_{f_i} : \ i = 1,\dots,m \Big\} = N & \\
%     &\textnormal{for every} \ X \in \Omega_g ,
% \end{align*}
where $\F_g$ is the family of vector fields \eqref{eq:vf_statlin}, which is generated by $F_{f_0,g} , F_{f_1} , \dots , F_{f_m}$, and $\Omega_g \subset \M \times \Sym^+(n)$ is an open and dense subset which depends on $g$ uniquely.
\end{corollary}

\begin{theorem}[Controllability with Respect to Generic Drift] \label{theo:Contr}
Let $m \ge 2$. There exists an open and dense (with respect to the Whitney topology) subset $\mathcal{O}_{\textnormal{Contr}} \subset C^{\infty}(\M;\mathbb{R}^{n \times m})$, such that for every $(f_1,\dots,f_m) \in \mathcal{O}_{\textnormal{Contr}}$, it holds
$$
\dim \lie_{(m,P)} (\F_{0}) = N , \quad \textnormal{for every} \ (m,P) \in \M \times \Sym^+(n) ,
$$
where $\F_{0}$ is the family of vector fields \eqref{eq:vf_statlin}, which is generated by $F_{f_1} , \dots , F_{f_m}$.
% $$
% \dim \textnormal{Lie}_X\Big\{ F_{f_1} , \dots , F_{f_m} \Big\} = N , \ \textnormal{for every} \ X \in \mathbb{R}^n \times \Sym(n)^{++}  .
% $$
\end{theorem}

Through the rank conditions provided above, one can deduce the structure of the reachable sets in free and fixed time of the statistical linearization, and thus generic accessibility and controllability properties for \eqref{eq:syslin}, by means of Lemma~\ref{lemma:Acc}--\ref{lemma:Contr}.

The rest of the section is devoted to proving these results. In particular, we prove Theorem \ref{theo:Acc} for $m = 1$ (the cases $m \ge 2$ trivially result from the latter), given that the proofs of Theorems \ref{theo:Acc+} and \ref{theo:Contr} follow the same line, though they are less pedagogical. Finally, since all our proofs develop along local analysis, without loss of generality we implicitly assume $\M = \R^n$ in what follows.

\subsection{Fundamental concepts from transversality theory}

Before jumping into the proof of Theorem \ref{theo:Acc}, we recall some useful concepts from algebraic geometry and transversality theory which are key to achieve the aforementioned proof, for which we mainly refer to \cite{Whitney1957,Bochnak1998,Martinet1970,Goresky1988}. In particular, for the sake of clarity in the exposition, we gathered the classical concepts of algebraic geometry we make use of in our proofs in Appendix \ref{sec:appendixWhitney}, so that in this subsection we may focus on transversality theory.

Since we set up $m = 1$ and $\M = \R^n$, throughout the following sections, for any given $\ell \in \mathbb{N}$ we consider the vector bundle of $\ell$-jets $J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})$, for which we implicitly adopt the following identification
\begin{equation} \label{eq:Identification}
    J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) \cong \mathbb{R}^{3 n + 2 n \sum^{\ell}_{i=1} {\scriptsize \left(\begin{array}{c}
    n + i - 1 \\
    i
\end{array}\right)}} ,
\end{equation}
which is achieved through some (global) trivialization mapping. In addition, if $(U,\varphi)$ is any local chart of $\mathbb{R}^n$ at $m \in \mathbb{R}^n$, for every $f_0 , f_1 \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$ the coordinates $j^{\ell}_{\varphi}(f_0,f_1)_m$ of the jet $j^{\ell}(f_0,f_1)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})$ with respect to $(U,\varphi)$ are denoted by
\begin{align*}
j^{\ell}_{\varphi}( f_0 , f_1 )_m = \bigg( \varphi(m) , \ &\varphi^{f_0}_0 , \varphi^{f_1}_0 , \\
&(\varphi^{f_0}_{1;\{i_1\}})_{0 \le i_1 \le n} , (\varphi^{f_1}_{1;\{i_1\}})_{0 \le i_1 \le n} , \\
&\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
&(\varphi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}})_{0 \le i_1 \le \dots \le i_{\ell} \le n} ,  (\varphi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}})_{0 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
where $(\varphi^{f_0}_j)_{0 \le i_1 \le \dots \le i_j \le n} , (\varphi^{f_1}_j)_{0 \le i_1 \le \dots \le i_j \le n} \in \mathbb{R}^{n {\scriptsize \left(\begin{array}{c}
    n + j - 1 \\
    j
\end{array}\right)}}$, for every $1 \le j \le \ell$.

\vspace{5pt}

From now on, we fix an integer $\ell \in \mathbb{N}$ (to be appropriately chosen later) and we introduce the product vector bundle
$$
\Pi_{\ell} : E_{\ell} = J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) \times_{\mathbb{R}^n} \Sym(n) \rightarrow \mathbb{R}^n ,
$$
for which we implicitly adopt the identification
\begin{equation} \label{eq:Identification1}
    E_{\ell} \cong \mathbb{R}^{3 n + \frac{n(n+1)}{2} + 2 n \sum^{\ell}_{i=1} {\scriptsize \left(\begin{array}{c}
    n + i - 1 \\
    i
\end{array}\right)}} ,
\end{equation}
through some (global) trivialization mapping. In particular, with a slight abuse of notation, we denote the elements of $E_{\ell}$ by
$$
\big( j^{\ell}(f_0,f_1)_m , P \big) \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) \times_{\mathbb{R}^n} \Sym(n) .
$$
Therefore, the projection
\begin{align*}
    \Proj_{J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})} : \ &E_{\ell} \rightarrow J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) \\
    &\big( j^{\ell}(f_0,f_1)_m , P \big) \mapsto j^{\ell}(f_0,f_1)_m
\end{align*}
is a well-defined and smooth vector bundle homomorphism.

The identifications \eqref{eq:Identification} and \eqref{eq:Identification1} allow us to introduce semi-algebraic sets $\mathcal{SA} \subset J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})$ and semi-algebraic sets $\mathcal{SA} \subset E_{\ell}$ (see Appendix \ref{sec:appendixWhitney}), and thus we can make use of the following key transversality result to prove Theorem \ref{theo:Acc}:

\begin{theorem}[Transversality Theorem for $E_{\ell}$, Proposition p. 38
of \cite{Goresky1988}] \label{theo:Transversality}
Let $\mathcal{SA} \subset J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})$ be a closed semi-algebraic set which satisfies
$$
\codim \mathcal{SA} \ge n + 1 .
$$
Then, the subset
$$
\mathcal{O}_{\mathcal{SA}} = \Big\{ (f_0,f_1) \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^{2 n}) : \ j^{\ell}(f_0,f_1) \cap \mathcal{SA} = \emptyset \Big\}
$$
is open and dense (w.r.t. the Whitney topology) in $C^{\infty}(\mathbb{R}^n;\mathbb{R}^{2 n})$.
\end{theorem}

Theorem \ref{theo:Transversality} results from combining Theorem \ref{theo:Whitney} with Thom's stratified transversality theorem (for details, see \cite[``Th\'eor\`eme 6.1'' and ``Remarque'' at page 175]{Martinet1970}).

\subsection{Proof of Theorem \ref{theo:Acc}}

Our proof of Theorem \ref{theo:Acc} is inspired by the proofs in \cite{Lobry1972,Bonnard1997,Chitour2006}, which consist of showing that specific \textit{bad sets} have arbitrarily large codimension. We introduce appropriate, non-trivial modifications to these proofs to address submersion singularities which are due to possibly non-transverse components. In particular, we introduce four bad sets $\mathcal{B}^1_{\ell}$, $\mathcal{B}^2_{\ell}$, $\mathcal{B}^3_{\ell}$, and $\mathcal{B}^4_{\ell}$ (see below). Although we could prove our result without explicitly considering $\mathcal{B}^1_{\ell}$, we introduced this latter on purpose to show how the classical transversality cunning in \cite{Lobry1972,Bonnard1997,Chitour2006}, which can be leveraged to handle $\mathcal{B}^1_{\ell}$, must be revisited to manipulate $\mathcal{B}^2_{\ell}$, $\mathcal{B}^3_{\ell}$, and $\mathcal{B}^4_{\ell}$.

\subsubsection{Definition of the bad sets} Through a slight abuse of notation which is possible thanks to the identifications \eqref{eq:Identification} and \eqref{eq:Identification1}, for $r \in \mathbb{N} \cap [0,\ell-2]$ the mappings
$$
\big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} \mapsto \ad^r F_{f_0,0} \cdot F_{f_1}(m,P) \in \mathbb{R}^N ,
$$
$$
\big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} \mapsto \ad^r \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(m,P) \in \mathbb{R}^N ,
$$
where $\ad^r$ is the $r$-iterated Lie bracket, are well-defined vector-valued polynomials. This remark, together with the identifications \eqref{eq:Identification} and \eqref{eq:Identification1}, allows us to defined the following bad sets, which are semi-algebraic sets of $E_{\ell}$ (for any $\ell \in \mathbb{N}$ large enough):
\begin{align*}
    \mathcal{B}^1_{\ell} = \bigg\{ &\big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} : \ f_0(m) \neq 0 , \ \det P \neq 0 , \\
    &\rank \Big[ \ad^1 F_{f_0,0} \cdot F_{f_1}(m,P) \ \Big| \ \ad^3 F_{f_0,0} \cdot F_{f_1}(m,P) \ \Big| \ \dots \\
    &\hspace{29ex} \dots \ \Big| \ \ad^{2 \lfloor \ell / 2 \rfloor - 1} F_{f_0,0} \cdot F_{f_1}(m,P) \Big] < N \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^2_{\ell} = \bigg\{ &\big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} : \ f_0(m) = 0 , \ \ad^1 f_0 \cdot f_1(m) \neq 0 , \ \det P \neq 0 , \\
    &\rank \Big[ \ad^1 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(m,P) \ \Big| \ \ad^3 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(m,P) \ \Big| \ \dots \\
    &\hspace{18ex} \dots \ \Big| \ \ad^{2 \lfloor (\ell - 1) / 2 \rfloor - 1} \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(m,P) \Big] < N \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^3_{\ell} = \bigg\{ &j^{\ell}(f_0,f_1)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) : \ f_0(m) = \ad^1 f_0 \cdot f_1(m) = 0 , \quad f_1(m) \neq 0 \bigg\} ,
\end{align*}
\begin{align*}
    \mathcal{B}^4_{\ell} = \bigg\{ &j^{\ell}(f_0,f_1)_m \in J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n}) : \ f_0(m) = f_1(m) = 0 \bigg\} ,
\end{align*}

Thanks to \eqref{eq:DimClosure} and \eqref{eq:DimProj}, we finally have that the bad set
$$
\mathcal{B}_{\ell} = \overline{\Proj_{J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})}( \mathcal{B}^1_{\ell} \cup \mathcal{B}^2_{\ell} ) \cup \mathcal{B}^3_{\ell} \cup \mathcal{B}^4_{\ell}} \subset J^{\ell}(\mathbb{R}^n;\mathbb{R}^{2 n})
$$
is a semi-algebraic set whose codimension satisfies
\begin{equation} \label{eq:TestCodim}
    \codim \mathcal{B}_{\ell} \ge \left\{\underset{i=1,2}{\max} \left\{ \codim \mathcal{B}^i_{\ell} - \frac{n(n+1)}{2} \right\} , \underset{i=3,4}{\max} \ \codim \mathcal{B}^i_{\ell} \right\} .
\end{equation}

\subsubsection{Existence of an open and dense subset}

Assume that
\begin{equation} \label{eq:ReqCodim}
    \underset{i=1,2}{\max} \ \codim \mathcal{B}^i_{\ell} \ge \frac{n(n+1)}{2} + n + 1 , \quad \underset{i=3,4}{\max} \ \codim \mathcal{B}^i_{\ell} \ge n + 1 , \quad \textnormal{for some} \ \ell \in \mathbb{N} .
\end{equation}
Therefore, \eqref{eq:TestCodim} yields $\codim \mathcal{B}_{\ell} \ge n + 1$ and we can apply Theorem \ref{theo:Transversality} to infer the existence of an open and dense (with respect to the Whitney topology) subset
$$
\mathcal{O}_{\textnormal{Acc}} = \Big\{ (f_0,f_1) \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^{2 n}) : \ j^{\ell}(f_0,f_1) \cap \mathcal{B}_{\ell} = \emptyset \Big\} \subset C^{\infty}(\mathbb{R}^n;\mathbb{R}^{2 n}) .
$$
In particular, straightforward computations by contradiction show that
$$
(f_0,f_1) \in \mathcal{O}_{\textnormal{Acc}} \ \Longrightarrow \ \dim \lie_{(m,P)} \left( \vecdef{f}{Df P + P Df^{\top}} \ : \ f \in \{ f_0 , f_1 \} \right) = N ,
$$
if $\det P \neq 0$. Therefore, the proof of Theorem \ref{theo:Acc} is achieved once \eqref{eq:ReqCodim} is proved.

\begin{remark}
Theorem \ref{theo:Acc+} may be proved similarly by replacing $\mathcal{B}^1_{\ell}$ with
\begin{align*}
    \bigg\{ &\big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} : \ f_0(m) \neq 0 , \ \ad^1 f_0 \cdot f_1(m) \neq 0 , \ \det P \neq 0 , \\
    &\rank \Big[ \ad^1 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \ \Big| \ \ad^3 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \ \Big| \ \dots \\
    &\hspace{18ex} \dots \ \Big| \ \ad^{2 \lfloor (\ell - 1) / 2 \rfloor - 1} \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \Big] < N \bigg\} .
\end{align*}
The required modifications are straightforward, and thus we avoid to report them.
\end{remark}

\subsubsection{Codimension computations}

The rest of the manuscript is devoted to prove \eqref{eq:ReqCodim}. We provide computations for $\mathcal{B}^1_{\ell}$ and $\mathcal{B}^2_{\ell}$ uniquely, given that the computations for $\mathcal{B}^3_{\ell}$ and $\mathcal{B}^4_{\ell}$ essentially follow the same line, though they are easier.

We fix $\ell \in \mathbb{N}$ large enough (to be selected later). For $r \in \mathbb{N}$, $m \in \mathbb{R}^n$, and $h_0 , \dots , h_r \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$, we denote by
$$
\big( D^r h_0 \big)_{i_1,\dots,i_r}(m) = \frac{\partial^r h_0}{\partial x_{i_1} \dots \partial x_{i_r}}(m) \in \mathbb{R}^n
$$
the tensor-valued mapping given by the $r$th derivative of $h_0$ with respect to the multi-index $(i_1,\dots,i_r)$, as well as the matrix-valued mapping
$$
\big( (D^{r+1} h_0) h_1 \dots h_r \big)_{i j}(m) = \sum^n_{i_1,\dots,i_r=1} \big( D^{r+1} h_0 \big)^i_{j,i_1,\dots,i_r}(m) h^{i_1}_1(m) \dots h^{i_r}_r(m) \in \mathbb{R}^{n \times n} .
$$
Also, we denote the symmetric tensorization of any element $\theta_r \in \mathbb{R}^{n {\scriptsize \left(\begin{array}{c}
    n + r - 1 \\
    r
\end{array}\right)}}$ by
$$
S(\theta_r) : \underbrace{\mathbb{R}^n \times \dots \times \mathbb{R}^n}_{r-\textnormal{times}} \rightarrow \mathbb{R}^n ,
$$
whereas denote the symmetrization of a matrix $A \in \mathbb{R}^n$ by $\Sym(A) = A + A^{\top}$. For every $r \in \mathbb{N}$ and $\rho \in [0,r]$, we denote by $L^{\rho}_r$ the Stiefel manifold of linear mappings
$$
L : \mathbb{R}^r \rightarrow \mathbb{R}^N
$$
such that $\rank L = \rho$, for which
\begin{equation} \label{eq:Stiefel}
    \codim L^{\rho}_r = \left( N - \rho \right) (r - \rho) .
\end{equation}
Finally, for every $r \in \mathbb{N}$, we introduce the notation $\bm{1}_r = (1,\dots,1) \in \mathbb{R}^r$.

\vspace{5pt}

\textbf{Computations for $\bm{\mathcal{B}^1_{\ell}}$.}

\vspace{5pt}

We introduce appropriate coordinates, i.e., the mapping $\chi$ defined below, under which it is easy to check that appropriate mappings are submersions, yielding the desired result. Note that the mapping $\chi$ has been first introduced in \cite[Section 5]{Bonnard1997}. Unfortunately, due to some Lie bracket singularities, the technique developed in \cite{Bonnard1997} does not work for $\mathcal{B}^2_{\ell}$, and we will need to introduce new singularity-free coordinates.

\vspace{5pt}

Straightforward computations by induction yield the following key result.

\begin{proposition} \label{Prop:FirstBrackets}
For $X = (m,P) \in \mathbb{R}^n \times \Sym(n)$ and $f_0 \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$ such that $f_0(m) \neq 0$, the following equivalence holds true for $f_1 \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$ and $r \in \mathbb{N}$:
\begin{align*}
    \ad^r F_{f_0,0} \cdot F_{f_1}(X) = \ &\left(\begin{array}{c}
        A_{r}\big( D^{i+1} f_0 , D^i f_1 , \ 0 \le i \le r-1 \big) \\[10pt]
        B_{r}\big( P , D^{i+1} f_0 , D^i f_1 , \ 0 \le i \le r \big)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        (D^r f_1) \underbrace{f_0 \dots f_0}_{r-\textnormal{times}} \\
        \Sym\bigg( \Big( (D^{r+1} f_1) \underbrace{f_0 \dots f_0}_{r-\textnormal{times}} \Big) P \bigg)
    \end{array}\right) ,
\end{align*}
where $A_r$ and $B_r$ are polynomial expressions of $P$ and of the derivatives of $f_0$ and $f_1$.
\end{proposition}

Consider the canonical global chart $(\mathbb{R}^n,Id)$ of $\mathbb{R}^n$, given by the identity map $Id$. Since every $\big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{B}^1_{\ell}$ satisfies $Id^{f_0}_0 \neq 0$ and $\det P \neq 0$, we may select constant vectors $v_2 , \dots , v_n \in \mathbb{R}^n$ such that the tuple of vectors
$$
\{ v_1(p) , v_2(p) , \dots , v_n(p) \} = \{ Id^{f_0}_0 , v_2 , \dots , v_n \} , \quad \textnormal{for} \  p = \big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{V}^1_{\ell} ,
$$
spans $\mathbb{R}^n$ in some open subset $\mathcal{V}^1_{\ell} \subset E_{\ell}$, and such that every $\big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{V}^1_{\ell}$ satisfies $\det P \neq 0$. In particular, the mapping
\begin{align*}
    \chi\Big( &\big( j^{\ell}(f_0,f_1)_m , P \big) \Big) = \bigg( \chi^m_0 = m , \quad \chi^P_0 = P , \\
    &\chi^{f_0}_0 = Id^{f_0}_0 , \quad \chi^{f_1}_0 = Id^{f_1}_0 , \\
    &\Big( \chi^{f_0}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} = \Big( S(Id^{f_0}_1) v_{i_1} \Big)_{1 \le i_1 \le n} , \\
    &\Big( \chi^{f_1}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} = \Big( S(Id^{f_1}_1) v_{i_1} \Big)_{1 \le i_1 \le n} , \\
    &\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
    &\Big( \chi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(Id^{f_0}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , \\
    &\Big( \chi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( S(Id^{f_1}_{\ell}) v_{i_1} \dots v_{i_{\ell}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
which is well-defined and smooth in $\mathcal{V}^1_{\ell}$, is a local chart for $E_{\ell}$. For $\big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{V}^1_{\ell}$, let $M$ denote the matrix which corresponds to the smooth change of coordinates
$$
P^j = \sum^n_{i=1} M_{ij}(\theta^{f_0}_0,P) v_i , \quad M(\theta^{f_0}_0,P) = \big( M_{ij}(\theta^{f_0}_0,P) \big)_{1 \le i , j \le n} \in GL(n) ,
$$
where $P^j$ denotes the $j$th column of $P$. Therefore, for $r \in \mathbb{N}$ we may compute
\begin{align*}
    (D^{r+1} \ &f_1) \underbrace{f_0 \dots f_0}_{r-\textnormal{times}} P = \left( S(Id^{f_1}_{r+1}) \underbrace{Id^{f_0}_0 \dots Id^{f_0}_0}_{r-\textnormal{times}} P^1 \Big| \ \dots \ \Big| S(Id^{f_1}_{r+1}) \underbrace{Id^{f_0}_0 \dots Id^{f_0}_0}_{r-\textnormal{times}} P^n \right) \\[10pt]
    &= \left( S(Id^{f_1}_{r+1}) \underbrace{v_1 \dots v_1}_{r-\textnormal{times}} v_1 \Big| S(Id^{f_1}_{r+1}) \underbrace{v_1 \dots v_1}_{r-\textnormal{times}} v_2 \Big| \ \dots \ \Big| S(Id^{f_0}_{r+1}) \underbrace{v_1 \dots v_1}_{r-\textnormal{times}} v_n \right) M \\[10pt]
    &= \Big( \chi^{f_1}_{r+1;\bm{1}_{r+1}} \Big| \chi^{f_1}_{r+1;\{\bm{1}_r,2\}} \Big| \ \dots \ \Big| \chi^{f_1}_{r+1;\{\bm{1}_r,n\}} \Big) M ,
\end{align*}
which together with the equivalence of Proposition \ref{Prop:FirstBrackets} finally yields
\begin{align} \label{eq:TransformedBracketFirst}
    \ad^r F_{f_0,0} \cdot \ &F_{f_1}(X) = \left(\begin{array}{c}
        A_{r}\big( \chi^{f_0}_{i+1} , \chi^{f_1}_i , \ 0 \le i \le r-1 \big) \\[10pt]
        B_{r}\big( \chi^P_0 , \chi^{f_0}_{i+1} , \chi^{f_1}_i , \ 0 \le i \le r \big)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        \chi^{f_1}_r \\
        \Sym\bigg( \Big( \chi^{f_1}_{r+1;\bm{1}_{r+1}} \Big| \chi^{f_1}_{r+1;\{\bm{1}_r,2\}} \Big| \ \dots \ \Big| \chi^{f_1}_{r+1;\{\bm{1}_r,n\}} \Big) M(\chi^{f_0}_0,\chi^P_0) \bigg)
    \end{array}\right) , \nonumber
\end{align}
for every $\big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{V}^1_{\ell}$ and every $r \in \mathbb{N} \cap [1,\ell-1]$.

At this step, up to appropriate identifications, the triangular form of \eqref{eq:TransformedBracketSecond} allows us to infer that, for every $\ell \in \mathbb{N}$ such that $2 \lfloor \ell / 2 \rfloor - 1 \ge N$, the mappings
\begin{align*}
    \mathcal{L}^1_{\ell} &= \rank \Big[ \ad^1 F_{f_0,0} \cdot F_{f_1}(X) \ \Big| \ \ad^3 F_{f_0,0} \cdot F_{f_1}(X) \ \Big| \ \dots \\
    &\hspace{20ex} \dots \ \Big| \ \ad^{2 \lfloor \ell / 2 \rfloor - 1} F_{f_0,0} \cdot F_{f_1}(X) \Big] : \ \mathcal{V}^1_{\ell} \rightarrow \mathbb{R}^{N \times (2 \lfloor \ell / 2 \rfloor - 1)}
\end{align*}
are submersions. In particular, we infer that $(\mathcal{L}^1_{\ell})^{-1}(L^{\rho}_{2 \lfloor \ell / 2 \rfloor - 1}) \subset \mathcal{V}^1_{\ell}$ are submanifolds for every $\rho \in [0,N]$, which due to \eqref{eq:Stiefel} satisfy
\begin{align} \label{eq:Stiefel1}
    \codim (\mathcal{L}^1_{\ell})^{-1}(L^{\rho}_{2 \lfloor \ell / 2 \rfloor - 1}) &= \codim L^{\rho}_{2 \lfloor \ell / 2 \rfloor - 1} \\
    &= \left( N - \rho \right) \Big( 2 \lfloor \ell / 2 \rfloor - 1 - \rho \Big) . \nonumber
\end{align}
Since
$$
\mathcal{B}^1_{\ell} \cap \mathcal{V}^1_{\ell} \subset \bigcup^{N - 1}_{\rho = 1} (\mathcal{L}^1_{\ell})^{-1}(L^{\rho}_{2 \lfloor \ell / 2 \rfloor - 1}) ,
$$
thanks to \eqref{eq:Stiefel1} we finally obtain that
\begin{align*}
    \codim \mathcal{B}^1_{\ell} \cap \mathcal{V}^1_{\ell} &\ge \codim (\mathcal{L}^1_{\ell})^{-1}\left( L^{N - 1}_{2 \lfloor \ell / 2 \rfloor - 1} \right) \\
    &= 2 \lfloor \ell / 2 \rfloor - n - \frac{n(n+1)}{2} \ge N + 1 ,
\end{align*}
as soon as we select $\ell \in \mathbb{N}$ large enough. We conclude that \eqref{eq:ReqCodim} holds true for $\mathcal{B}^1_{\ell}$.

\vspace{5pt}

\textbf{Computations for $\bm{\mathcal{B}^2_{\ell}}$.}

\vspace{5pt}

Unfortunately, the technique developed in the previous section does not work for $\mathcal{B}^2_{\ell}$, in that the Lie bracket $\ad^1 f_0 \cdot f_1$ is trivial. Thus, we introduce new singularity-free coordinates, i.e., the mapping $\psi$ defined below, which allow us to easily show surjectivity of some differentials, yielding the desired result also in this singular case.

\vspace{5pt}

We start proving the existence of new singularity-free coordinates enabling the following key equivalence between high-order Lie brackets.

\begin{proposition} \label{Prop:SecondBrackets}
For every $X = (m,P) \in \mathbb{R}^n \times \Sym(n)$ and every $f_0 , f_1 \in C^{\infty}(\mathbb{R}^n;\mathbb{R}^n)$ satisfying $\ad^1 f_0 \cdot f_1(m) \neq 0$, there exists a local chart $(U,\varphi)$ of $\mathbb{R}^n$ at $m$ which smoothly depends on the coefficients of both $f_0$ and $f_1$, and such that for every $r \in \mathbb{N}$, the following equivalence holds true:
\begin{align*}
    \ad^r \big[ F_{f_0,0} , F_{f_1} \big] \cdot \ &F_{f_1}(X) = \left(\begin{array}{c}
        0 \\[10pt]
        \displaystyle \Sym\left( (D^2 \varphi^{-1}) \frac{\partial^r f_1}{\partial^r x^{\varphi}_1} D\varphi P \right)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        \displaystyle D \varphi^{-1} \frac{\partial^r f_1}{\partial^r x^{\varphi}_1} \\[10pt]
        \displaystyle \Sym\left( D \varphi^{-1} \left( \frac{\partial^{r+1} f_1}{\partial^{r+1} x^{\varphi}_1} \ \bigg| \ \frac{\partial^{r+1} f_1}{\partial^r x^{\varphi}_1 x^{\varphi}_2} \ \bigg| \ \dots \ \bigg| \ \frac{\partial^{r+1} f_1}{\partial^r x^{\varphi}_1 x^{\varphi}_n} \right) D \varphi P \right)
    \end{array}\right) .
\end{align*}
\end{proposition}

\begin{proof}[Proof of Proposition \ref{Prop:SecondBrackets}]
We first start by recalling a classic representation result, in a general abstract framework. Let $M$ be a $n$-dimensional manifold, and $V \in C^{\infty}(M;TM)$ be a smooth vector field, i.e., a section of the tangent bundle $\pi_M : TM \to M$. Fix $p \in M$, and let $(U_1,\varphi)$ and $(U_2,\psi)$ be local charts of $M$ at $p$, so that
$$
\tilde \varphi\left( p , \sum^n_{i=1} v_i \partial^{\varphi}_i(p) \right) = (\varphi(p) , v) , \quad \tilde \psi\left( p , \sum^n_{i=1} w_i \partial^{\psi}_i(p) \right) = (\varphi(p) , w)
$$
are local charts for $TM$ with domains $\pi^{-1}_M(U_1)$ and $\pi^{-1}_M(U_2)$, respectively. If
$$
\sum^n_{i=1} V^{\varphi}_i(p) \partial^{\varphi}_i(p) = V(p) = \sum^n_{i=1} V^{\psi}_i(p) \partial^{\psi}_i(p) ,
$$
the following rules for the change of coordinates of $V$ and its differential, hold:
\begin{equation} \label{eq_change1}
    V^{\psi}(p) = D\big( \psi \circ \varphi^{-1} \big)(p) V^{\varphi}(p) ,
\end{equation}
\begin{equation} \label{eq_change2}
    D\big( \tilde \psi \circ V \circ \psi^{-1} \big)(p) = D\big( \tilde \psi \circ \tilde \varphi^{-1} \big)(p,V(p)) D\big( \tilde \varphi \circ V \circ \varphi^{-1} \big)(p) D\big( \varphi \circ \psi^{-1} \big)(p) ,
\end{equation}
with
$$
D\big( \tilde \psi \circ \tilde \varphi^{-1} \big)(p,V(p)) = \left(\begin{array}{cc}
    D\big( \psi \circ \varphi^{-1} \big)(p) & 0 \\[10pt]
    D^2\big( \psi \circ \varphi^{-1} \big) V^{\varphi}(p) & D\big( \psi \circ \varphi^{-1} \big)(p)
\end{array}\right) \in GL(2 n) .
$$

At this step, since $\ad^1 f_0 \cdot f_1(m) \neq 0$ we may find a local chart $(U,\varphi)$ of $\mathbb{R}^n$ at $m$, which smoothly depends on the coefficients of both $f_0$ and $f_1$ (indeed, this chart is a smooth mapping of the flow of the vector field $\ad^1 f_0 \cdot f_1$, which is smooth with respect to the coefficients of both $f_0$ and $f_1$), and such that
$$
[ f_0 , f_1 ] = \partial^{\varphi}_1 , \quad \textnormal{locally in} \ U .
$$
In these coordinates, through straightforward computations, we obtain
$$
( \ad^r [ f_0 , f_1 ] \cdot f_1 )^{\varphi} = \frac{\partial^r f_1}{\partial^r x^{\varphi}_1} , \quad \textnormal{locally in} \ U ,
$$
and therefore, by selecting $M = \mathbb{R}^n$, $V = \ad^r [ f_0 , f_1 ] \cdot f_1$, $(U_1,\varphi) = (U,\varphi)$, and $(U_2,\psi) = (\mathbb{R}^n,Id)$, the relations \eqref{eq_change1} and \eqref{eq_change2} respectively yield
$$
\ad^r [ f_0 , f_1 ] \cdot f_1 = D \varphi^{-1} \frac{\partial^r f_1}{\partial^r x^{\varphi}_1} , \quad \textnormal{locally in} \ U ,
$$
\begin{align*}
    &D\big( \ad^r [ f_0 , f_1 ] \cdot f_1 \big) = (D^2 \varphi^{-1}) \frac{\partial^r f_1}{\partial^r x^{\varphi}_1} D\varphi \\
    &+ D \varphi^{-1} \left( \frac{\partial^{r+1} f_1}{\partial^{r+1} x^{\varphi}_1} \ \bigg| \ \frac{\partial^{r+1} f_1}{\partial^r x^{\varphi}_1 x^{\varphi}_2} \ \bigg| \ \dots \ \bigg| \ \frac{\partial^{r+1} f_1}{\partial^r x^{\varphi}_1 x^{\varphi}_n} \right) D \varphi , \quad \textnormal{locally in} \ U ,
\end{align*}
and the conclusion readily follows from Lemma \ref{lem:LieBrac}.
\end{proof}

Let us introduce the subset
$$
\mathcal{S}^2_{\ell} = \bigg\{ \big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} : \ f_0(m) = 0 , \ \ad^1 f_0 \cdot f_1(m) \neq 0 , \ \det P \neq 0 \bigg\} .
$$
Since the mapping
$$
\mathcal{F}^2_{\ell} : \ E_{\ell} \rightarrow \mathbb{R}^n : \ \big( j^{\ell}(f_0,f_1)_m , P \big) \mapsto f_0(m)
$$
is a submersion, we infer that
$$
\mathcal{S}^2_{\ell} = ( \mathcal{F}^2_{\ell} )^{-1}(0) \setminus \Big\{ \big( j^{\ell}(f_0,f_1)_m , P \big) \in E_{\ell} : \ \ad^1 f_0 \cdot f_1(m) = 0 \ \textnormal{or} \ \det P = 0 \Big\}
$$
is an embedded submanifold of $E_{\ell}$ with $\dim \mathcal{S}^2_{\ell} = \dim E_{\ell} - n$, which contains $\mathcal{B}^2_{\ell}$. By fixing $m \in \mathbb{R}^n$ and letting $(U,\varphi)$ be the local chart of $\mathbb{R}^n$ at $m$ given by Proposition \ref{Prop:SecondBrackets}, which smoothly depends on the coefficients of both $f_0$ and $f_1$, we define the open set $\mathcal{V}^2_{\ell} = \Pi^{-1}_{\ell}(U) \subset E_{\ell}$. Therefore, the mapping
\begin{align*}
    \psi\Big( \big( j^{\ell}(f_0,f_1)_m , \ &P \big) \Big) = \bigg( \psi^m_0 = \varphi(m) , \quad \psi^P_0 = D \varphi(m) P , \\
    &\psi^{f_0}_0 = D \varphi^{-1}(m) \varphi^{f_0}_0 , \quad \psi^{f_1}_0 = D \varphi^{-1}(m) \varphi^{f_1}_0 , \\
    &\Big( \psi^{f_0}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} = \Big( D \varphi^{-1}(m) \varphi^{f_0}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} , \\
    &\Big( \psi^{f_1}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} = \Big( D \varphi^{-1}(m) \varphi^{f_1}_{1;\{i_1\}} \Big)_{1 \le i_1 \le n} , \\
    &\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots \\
    &\Big( \psi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( D \varphi^{-1}(m) \varphi^{f_0}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} , \\
    &\Big( \psi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} = \Big( D \varphi^{-1}(m) \varphi^{f_1}_{\ell;\{i_1,\dots,i_{\ell}\}} \Big)_{1 \le i_1 \le \dots \le i_{\ell} \le n} \bigg) ,
\end{align*}
which is well-defined and smooth in $\mathcal{V}^2_{\ell}$, is a local chart for $E_{\ell}$ which is adapted to $\mathcal{S}^2_{\ell}$. Finally, evaluating the equivalence of Proposition \ref{Prop:SecondBrackets} through this chart yields
\begin{align} \label{eq:TransformedBracketSecond}
    \ad^r \big[ F_{f_0,0} , F_{f_1} \big] \cdot \ &F_{f_1}(X) = \left(\begin{array}{c}
        0 \\[10pt]
        \displaystyle \Sym\left( (D^2 \varphi^{-1})(\psi^m_0) D \varphi\big( \varphi^{-1}(\psi^m_0) \big) \psi^{f_1}_{r;\bm{1}_r} \psi^P_0 \right)
    \end{array}\right) \\[10pt]
    &+ \left(\begin{array}{c}
        \displaystyle \psi^{f_1}_{r;\bm{1}_r} \\[10pt]
        \displaystyle \Sym\bigg( \Big( \psi^{f_1}_{r+1;\bm{1}_{r+1}} \ \Big| \ \psi^{f_1}_{r+1;\{\bm{1}_r,2\}} \ \Big| \ \dots \ \Big| \ \psi^{f_1}_{r+1;\{\bm{1}_r,n\}} \Big) \psi^P_0 \bigg)
    \end{array}\right) , \nonumber
\end{align}
for every $\big( j^{\ell}(f_0,f_1)_m , P \big) \in \mathcal{S}^2_{\ell} \cap \mathcal{V}^2_{\ell}$ and every $r \in \mathbb{N} \cap [0,\ell-2]$.

At this step, up to appropriate identifications, the triangular form of \eqref{eq:TransformedBracketSecond} allows us to infer that, for every $\ell \in \mathbb{N}$ such that $2 \lfloor (\ell - 1) / 2 \rfloor - 1 \ge N$, the mappings
\begin{align*}
    \mathcal{L}^2_{\ell} &= \rank \Big[ \ad^1 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \ \Big| \ \ad^3 \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \ \Big| \ \dots \\
    &\dots \ \Big| \ \ad^{2 \lfloor (\ell - 1) / 2 \rfloor - 1} \big[ F_{f_0,0} , F_{f_1} \big] \cdot F_{f_1}(X) \Big] : \ \mathcal{S}^2_{\ell} \cap \mathcal{V}^2_{\ell} \rightarrow \mathbb{R}^{N \times (2 \lfloor (\ell - 1) / 2 \rfloor - 1)}
\end{align*}
are submersions. In particular, we infer that $(\mathcal{L}^2_{\ell})^{-1}(L^{\rho}_{2 \lfloor (\ell - 1) / 2 \rfloor - 1}) \subset \mathcal{S}^2_{\ell} \cap \mathcal{V}^2_{\ell}$ are submanifolds for every $\rho \in [0,N]$, which due to \eqref{eq:Stiefel} satisfy
\begin{align} \label{eq:Stiefel2}
    \codim (\mathcal{L}^2_{\ell})^{-1}(L^{\rho}_{2 \lfloor (\ell - 1) / 2 \rfloor - 1}) &= \codim L^{\rho}_{2 \lfloor (\ell - 1) / 2 \rfloor - 1} \\
    &= \left( N - \rho \right) \Big( 2 \lfloor (\ell - 1) / 2 \rfloor - 1 - \rho \Big) . \nonumber
\end{align}
Since
$$
\mathcal{B}^2_{\ell} \cap \mathcal{V}^2_{\ell} \subset \bigcup^{N - 1}_{\rho = 1} (\mathcal{L}^2_{\ell})^{-1}(L^{\rho}_{2 \lfloor (\ell - 1) / 2 \rfloor - 1}) ,
$$
thanks to \eqref{eq:Stiefel2} we finally obtain that
\begin{align*}
    \codim \mathcal{B}^2_{\ell} \cap \mathcal{V}^2_{\ell} &\ge \codim (\mathcal{L}^2_{\ell})^{-1}\left( L^{N - 1}_{2 \lfloor (\ell - 1) / 2 \rfloor - 1} \right) \\
    &= 2 \lfloor (\ell - 1) / 2 \rfloor - n - \frac{n(n+1)}{2} \ge N + 1 ,
\end{align*}
as soon as we select $\ell \in \mathbb{N}$ large enough. We conclude that \eqref{eq:ReqCodim} holds true for $\mathcal{B}^2_{\ell}$.

This latter argument concludes the proof of Theorem \ref{theo:Acc}.

% \begin{remark}[Obstruction for $m < 2$ in the previous proof]
% The key step in the previous proof consists of proving that the mappings $\mathcal{L}^{\ell}_q$ are submersions for every $\ell \ge N$, which in turn relies on the alternate triangular selection \eqref{eq:TriangularSelection}. Unfortunately, when $m < 2$, it is no longer possible to leveraging alternate triangular selections \eqref{eq:TriangularSelection}, hindering the validity of Theorem \ref{theo:Acc}, \ref{theo:Acc0}, \ref{theo:Contr}, and of Corollary \ref{coroll:Acc}.

% Indeed, if we were to replicate the previous steps for $m < 2$, we would need to prove that, for every $\ell \ge N$, the mappings
% \begin{align*}
%     \mathcal{G}^{\ell}_q = \rank \Big[ &\ad^0 F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \ad^1 F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \\
%     &\ad^2 F_{f_0,g} \cdot F_{f_1}(X) \ \Big| \ \dots \ \Big| \ \ad^{\ell} F_{f_0,g} \cdot F_{f_1}(X) \Big] : \ \mathcal{S}^2_{\ell} \cap \mathcal{U}_q \rightarrow \mathbb{R}^{\left( N \right) \times \ell}
% \end{align*}
% are submersions. By considering the simplest case in which the vectors $f_0$ and $f_1$ are linearly independent, and by appropriately upgrading the definitions of $\mathcal{S}^2_{\ell}$, $\psi$, and $\mathcal{U}_q$, the $r$-column of each mapping $\mathcal{G}^{\ell}_q$ would now be of the form
% \begin{equation} \label{eq:NewMapping}
%     \left(\begin{array}{c}
%         \psi^{f_1}_{r;\bm{1}_r} - \psi^{f_0}_{r;\{\bm{1}_{r-1},2\}} \\
%         \hspace{-33ex}\Sym\Bigg( \bigg( \Big( \psi^{f_1}_{r+1;\{\bm{1}_r,1\}} \Big| \ \dots \ \Big| \psi^{f_1}_{r+1;\{\bm{1}_r,n\}} \Big) \\
%         \hspace{10ex}- \Big( \psi^{f_0}_{r+1;\{\bm{1}_{r-1},1,2\}} \Big| \psi^{f_0}_{r+1;\{\bm{1}_{r-1},2,2\}} \Big| \ \dots \ \Big| \psi^{f_0}_{r+1;\{\bm{1}_{r-1},2,n\}} \Big) \bigg) M \Bigg)
%     \end{array}\right) ,
% \end{equation}
% where $M = M(\psi^{f_0}_0,\psi^{f_1}_0,P)$ is a smooth invertible matrix. In such situation, it is not difficult to see that \eqref{eq:NewMapping} implies that the image of
% $$
% d \mathcal{G}^{\ell}_q(p) : T_p \big( \mathcal{S}^2_{\ell} \cap \mathcal{U}_q \big) \rightarrow \mathbb{R}^{\left( N \right) \times \ell} , \quad p \in \mathcal{S}^2_{\ell} \cap \mathcal{U}_q ,
% $$
% has codimension
% $$
% \codim d \mathcal{G}^{\ell}_q(p) \Big( T_p \big( \mathcal{S}^2_{\ell} \cap \mathcal{U}_q \big) \Big) \ge 1 ,
% $$
% and thus $\mathcal{G}^{\ell}_q$ are not submersions. Moreover, the mappings $\mathcal{G}^{\ell}_q$ are not in general transverse to the Stiefel manifolds $L^{\rho}_{n,\ell}$. In conclusion, in this case we can not infer whether $(\mathcal{G}^{\ell}_q)^{-1}(L^{\rho}_{n,\ell}) \subset \mathcal{S}^2_{\ell} \cap \mathcal{U}_q$ are submanifolds for every $\rho \in [0,\ell]$.

% Note that alternatively considering Lie brackets of the type
% $$
% [F_{f_0,g} , \dots , [ F_{f_1} , [F_{f_0,g} , F_{f_1} ] ] \dots ]
% $$
% does not really help, especially when the vector fields $f_0$ and $f_1$ are linearly dependent.
% \end{remark}
